Stabilization of $866$ nm laser with Pound-Drever-Hall (PDH) technique for quantum manipulation of Ca+ ion in Paul trap

This article provides an introduction to one of the most efficient laser stabilization techniques - the Pound-Drever-Hall (PDH) method. The aim of the experiment is to build the PDH stabilization apparatus from scratch. I describe all the necessary theoretical treatment to formulate the technique and then describe it as I have experimentally implemented in the lab. All major sources of noise are discussed and noise tackling methods are implemented. All the equipments used are also described in detail for their principle and working.

==> Chapters/01_Abstract.tex <==
%
% Abstract.tex

\textbf{This article provides an introduction to one of the most efficient laser stabilization techniques - the Pound-Drever-Hall (PDH) method. I describe all the necessary theoretical treatment to formulate the technique and then describe it as I have experimentally implemented in the lab. All major sources of noise are discussed and noise tackling methods are implemented. All the equipments used are also described in detail for their principle and working.}




